Orbital dynamics and spin-precession around a circular chiral vorton

Vortons are of interest in high-energy physics as possible dark matter candidates and as probes of Grand Unified Theories. Using the recently derived weak-field metric for a chiral vorton, we study the dynamics of test particles by analyzing both timelike and null geodesics. We identify several classes of trajectories, including bound precessing orbits, circular orbits, toroidal, and crown-type oscillations, as well as unbound scattering paths. Poincare surfaces of section reveal transitions between regular and chaotic motions that depend sensitively on the vorton tension $G\mu$ and initial conditions. We further compute the Lense-Thirring and general spin-precession frequencies for gyroscopes along Killing trajectories. The resulting precession profiles exhibit several distinct features not present in Kerr black holes but reminiscent of Kerr naked singularities, such as: divergences near the ring core, and multi-minima structures. These dynamical and precessional signatures may offer potential observational pathways for detecting vortons.

==> bibs.tex <==
\bibitem{PhysRevLett.82.1201_Heliumvortexlines}
G.~A.~Williams,
``Vortex-Loop Phase Transitions in Liquid Helium, Cosmic Strings, and High- ${T}_{c}$ Superconductors,''
Phys. Rev. Lett. \textbf{82}, 1201--1204 (1999)

\bibitem{witten1985superconducting}
E.~Witten,
``Cosmic Superstrings,''
Phys. Lett. B \textbf{153}, 243--246 (1985)

\bibitem{Jiao_2023_earlymatterstrings}
H.~Jiao, R.~Brandenberger and A.~Refregier,
``Early Structure Formation from Cosmic String Loops in Light of Early JWST Observations,''
Phys. Rev. D \textbf{108}, 2470--0029 (2023)

\bibitem{witten1985superconducting}
E.~Witten,
``Superconducting Strings,''
Nuclear Physics B \textbf{249}, 557--592 (1985)

\bibitem{Brandenberger_1996}
R.~Brandenberger, B.~Carter, A.~C.~Davis and M.~Trodden,
``Cosmic vortons and particle physics constraints,''
Phys. Rev. D \textbf{54}, 6059--6071 (1996)

\bibitem{Auclair_2021_vortondarkmatter}
P.~Auclair, P.~Peter, C.~Ringeval and D.~Steer, ,
``Irreducible cosmic production of relic vortons,''
Journal of Cosmology and Astroparticle Physics \textbf{2021}, 098 (2021)

\bibitem{de_Laix_1996_lensingcosmicstringloop}
A.~A.~de Laix and T.~Vachaspati,
``Gravitational lensing by cosmic string loops,''
Phys. Rev. D \textbf{54}, 4780--4791 (1996)

\bibitem{de_Laix_1996_lensingcosmicstringloop}
A.~A.~de Laix and T.~Vachaspati,
``Gravitational lensing by cosmic string loops,''
Phys. Rev. D \textbf{54}, 4780--4791 (1996)

\bibitem{hartmann2011detection}
A.~A.~de Laix and T.~Vachaspati,
``Detection of cosmic superstrings by geodesic test particle motion,''
Phys. Rev. D \textbf{83}, 045027 (2011)

\bibitem{hartmann2011detection}
B.~Hartmann, C.~L{\"a}mmerzahl and P.~Sirimachan,
``Detection of cosmic superstrings by geodesic test particle motion,''
Phys. Rev. D \textbf{83}, 045027 (2011)

\bibitem{Hartmann_2010}
B.~Hartmann and P.~Sirimachan,
``Geodesic motion in the space-time of a cosmic string,''
Journal of High Energy Physics \textbf{2010} (2011), 045027

\bibitem{Hartmann_2012}
B.~Hartmann and F.~Michel,
``Geodesic motion in the space-time of a cosmic string,''
Phys. Rev. D \textbf{86} (2012), 105026

\bibitem{putra2024gravitationalfieldlensingcircular}
L.~B.~Putra and H.~S.~Ramadhan,
``Gravitational field and lensing of a circular chiral vorton,''
Gen.Rel.Grav. \textbf{57} (2025) 6, 97

\bibitem{Chakraborty_2017_distinguishingKerrandNaked}
C.~Chakraborty, P.~Kocherlakota, M.~Patil, S.~Bhattacharyya, P.~S.~Joshi, A.~Królak,
``Distinguishing Kerr naked singularities and black holes using the spin precession of a test gyro in strong gravitational fields,''
Phys. Rev. D \textbf{95} (2017), 084024

\bibitem{Mc_Manus_1993}
D.~J.~Mc Manus and M.~A.~Vandyck,
``Weak-field gravity of revolving circular cosmic strings,''
Phys. Rev. D \textbf{47} no.4 (1993), 1491

\bibitem{broucke2005dynamicsElipeRing}
R.~Broucke and A.~Elipe,
``The dynamics of orbits in a potential field of a solid circular ring,''
Regular and Chaotic Dynamics \textbf{10} no.2, 129--143 (2005) 

\bibitem{Cao:2024pdb_chaotic_motion_swirl_univer}
Cao et al,
``Chaotic motion of particles in the spacetime of a Kerr black hole immersed in swirling universes,''
Eur. Phys. J. C \textbf{85} no.1, (2025) 

\bibitem{PhysRevD.109.064042_geod_motion_swirl_universe}
R.~Capobianco, B.~Hartmann and J.~Kunz
``Geodesic motion in a swirling universe: The complete set of solutions,''
Phys. Rev. D \textbf{109}, (2025) 

\bibitem{Wu_hairykerrprecession_2023}
M.~H.~Wu, H.~Guo and X.~M.~Kuang,
``Precession and Lense-Thirring effect of hairy Kerr spacetimes,''
Phys. Rev. D \textbf{107} no.6 (2023), 064033

\bibitem{PhysRevD.45.1840}
T.~Damour and J.~H.~Taylor,
``Strong-field tests of relativistic gravity and binary pulsars,''
Phys. Rev. D \textbf{45} no.6, 1840--1868 (1992)

\bibitem{Rezania_2003}
V.~Rezania,
``On the precession of the isolated pulsar PSR B1828-11: A time-varying magnetic field,''
Astronomy \& Astrophysics \textbf{339}, no.2, 653--658 (2003)

\bibitem{Link_2001}
B.~Link and R.~I.~Epstein
``Precession Interpretation of the Isolated Pulsar PSR B1828−11,''
The Astrophysical Journal \textbf{556}, no.1, 392--398 (2001)

\bibitem{Ashton_2017}
G.~Ashton, D.~I.~Jones and R.~Prix
``On the free-precession candidate PSR B1828-11: Evidence for increasing deformation,''
Monthly Notices of the Royal Astronomical Society, (2017)

\bibitem{Meng_2024}
Meng et al,
``The Relativistic Spin Precession in the Compact Double Neutron Star System PSR J1946+2052,''
The Astrophysical Journal \textbf{966}, no.1, (2024)

\bibitem{Venkatraman_Krishnan_2019}
Meng et al,
``Relativistic Spin Precession in the Binary PSR J1141−6545,''
The Astrophysical Journal Letters \textbf{873}, no.2, (2019)

